On exceptional Enriques surfaces

We give a complete description of all classical Enriques surfaces with non-zero global vector fields. In particular we show that there are such surfaces. The obtained result also applies to supersingular Enriques surfaces fulfilling a rather special condition. During this classification we study some properties of genus 1-fibrations special to characteristic as well as make a close study of the genus 1-fibration on the surfaces that we classify.

==> Dynkin.tex <==
%%   This package draws the Dynkin and extended Dynkin graphs in the
%%   simply laced case (A, D and E) with the exception of the A~ class.
%%   The appropriate control sequences are \dynkinA, \dynkinD, \dynkinE,
%%   \dynkinDtilde, and \dynkinEtilde. They all take a numerical argument
%%   which is separated with a space from following text. The vertices of the
%%   graphs are drawn with a macro \dynkinball which can be redefined by the
%%   user. See the option dotchoice below for details.
%%   
%%       There are several options, which all are set by the \setdynkin macro:
%%   
%%   \setdynkin size=.5cm<space> 
%%   
%%     sets the length of the horisontal and vertical edges. Any dimension
%%     specification acceptable by TeX is allowed where .5cm was put in the
%%     example. 1 cm is the default.
%%   
%%   \setdynkin slope="25<space>
%%   
%%     sets the characters of the line10 font to use for sloped edges in D and
%%     D~.  The argument, here "25, is the character for upwards slope and the
%%     corresponding for downwards slope is computed by adding 64 to it (which
%%     seems to be line10's encoding). The default value is 0.
%%   
%%   \setdynkin lines=1<space>
%%   
%%     sets the number of lines to use for the sloped edges. Currently only 1 or
%%     2 are possible and 2 is the default.
%%   
%%   \setdynkin dotchoice=y<space>
%%   
%%     sets whether or not it should be possible to use different types of
%%     vertices at different positions. The choices are y for yes and n for no
%%     (the default).  If y is set then the \dynkinball should take one argument
%%     and the graph drawing macros \dynkinA etc will take more than the numeric
%%     arguments. More precisely:
%%   
%%       If dotchoice is set and tags is not (see below) then the supplementary
%%       argument is a space-separated list of items, one for each vertex of the
%%       graph. These items then passed to the macro \dynkinball which then
%%       decides what type of edge to draw. The order in which the edges are
%%       drawn is as follows:
%%            For A the vertices are drawn form left to right.
%%            For D the vertices on the horisontal line are drawn 
%%          from left to right, then the upper vertex of the right 
%%          fork and finally the lower vertex of that fork.
%%            For D~ the the upper vertex of the left fork is drawn 
%%          first, then the lower vertex of that fork is drawn, then 
%%          the vertices on the horisontal line from left to right, 
%%          then the upper vertex of the right fork and finally the
%%          lower vertex of that fork.
%%            For E and  E~ the vertices are drawn from left to right
%%          and from the bottom to the top. Thus for E, for instance,
%%          first three vertices on the horisontal line are drawn,
%%          then the uppermost vertex and then finally the rest of 
%%          horisontal vertices.
%%       If dotchoice and tags is set then the supplementary arguement
%%       is a space-separated list of pairs of items, one such pair for each 
%%       vertex, the items are separated by a comma and the first item is
%%       passed to \dynkinball and the second will be placed near the edge
%%       on the drawn graph.
%%   
%%       Example:
%%         \setdynkin dotchoice=y \setdynkin tags=y
%%         \dynkinE 8 c,1 b,2 c,3 b,4 c,5 b,6 c,7 b,8
%%       This will mark the vertices with consecutive numbers and
%%       consecutively pass c, b, c, b, c, b, c, and b to \dynkinball.
%%   
%%     Note that the package will call \dynkinball once before actually
%%     drawing anything with the first item as argument and use that
%%     result to determine the extent of all the vertices. Hence it is
%%     not a good idea to make the vertices of different size.
%%     Three \dynkinball macros are provided. See \setdynkin ball below.
%%   
%%   \setdynkin tags=y<space>
%%   
%%     sets whether or not tags should be put close to each vertex. The
%%     arguments are y for yes and n for no (the default). The tags
%%     are specified as a space-separated list. When dotchoice is also
%%     the format for that list has already been described, when not the
%%     items are simply used.
%%   
%%   \setdynkin ball=bullet<space>
%%   
%%    sets \dynkinball to one of three predefined macros. The possibilities
%%    are
%%      ball=bullet  (the default)
%%       will set \dynkinball to a parameterless macro which produces a
%%       bullet ($\bullet$).
%%      ball=bulletandcirc
%%       will set  \dynkinball to a macro taking one argument which
%%       produces a bullet if the argument is b and a circle ($\circ$)
%%       if the argument is a c.
%%      ball=bigcirc
%%       will set \dynkinball to a parameterless macro which produces a
%%       big circle ($\bigcirc$).
%%    (Note that in all cases the box in which these characters are put
%%    is slightly bigger than the characters themselves which forces
%%    some adjustment as can be seen from the macros.

\catcode`\@=11
\let\e@\expandafter
\def\d@nkinsize{1cm}
\newcount\d@nkincount
\d@nkincount"00
\newif\if@ne

\def\LINE{\hbox to \hsize}
\def\setdynkin#1=#2 {\csname d@nkin@#1\endcsname{#2}}
\def\d@nkin@size#1{\def\d@nkinsize{#1}}
\def\d@nkin@slope#1{\d@nkincount#1}
\def\d@nkin@lines#1{\ifnum#1=1\@netrue\else\@nefalse\fi}
\newif\ifd@dotchoice
\newif\ifd@tags
\def\d@nkin@dotchoice#1{\if#1y\d@dotchoicetrue\else\d@dotchoicefalse\fi
\d@setdots}
\def\d@nkin@tags#1{\if#1y\d@tagstrue\else\d@tagsfalse\fi\d@setdots}
\def\d@setdots{%
\ifd@dotchoice
\def\d@nkinball{\e@\dynkinball\e@{\the\t@@@}}%
\ifd@tags
 \let\d@loopargs\d@loopargsa
 \let\count@rg\count@rga
 \let\init@rg\init@rga
 \let\pr@pare\pr@parea
\else
 \let\d@loopargs\d@loopargsbc
 \let\count@rg\count@rgbc
 \let\init@rg\init@rgbc
 \let\pr@pare\pr@pareb
\fi
\else
\def\d@nkinball{\dynkinball}%
\ifd@tags
 \let\d@loopargs\d@loopargsbc
 \let\count@rg\count@rgbc
 \let\init@rg\init@rgbc
 \let\pr@pare\pr@parec
\else
 \let\d@loopargs\d@loopargsd
 \let\count@rg\count@rgd
 \let\init@rg\init@rgd
 \let\pr@pare\pr@pared
\fi
\fi}

\def\d@nkin@ball#1{\e@\let\e@\dynkinball\csname d@nkin#1\endcsname}

\def\spl@ttoksa#1\@t#2\@t#3\t@end{\t@@@={#1}\t@@@@={#2}\global\t@@={#3}}%
\def\spl@ttoksb#1\@t#2\t@end{\t@@@={#1}\t@@@@={}\global\t@@={#2}}%
\def\spl@ttoksc#1\@t#2\t@end{\t@@@={}\t@@@@={#1}\global\t@@={#2}}%

\def\pr@parea{\e@\spl@ttoksa\the\t@@\t@end}%
\def\pr@pareb{\e@\spl@ttoksb\the\t@@\t@end}%
\def\pr@parec{\e@\spl@ttoksc\the\t@@\t@end}%
\def\pr@pared{\t@@{}\t@@@{}}%

\def\n@metop{\hbox to 0pt{\kern-\d@nkinrightdim\vbox to
\wd0{\vss\offinterlineskip\hsize\ht0\pr@pare
\centerline{\the\t@@@@}\kern2pt\d@nkinball}\hss}}%
%
\def\n@medown{\hbox to 0pt{\kern-\d@nkinrightdim%
\vtop to \wd0{\offinterlineskip\hsize\ht0\pr@pare%
\d@nkinball\kern2pt\centerline{\the\t@@@@}\vss}\hss}}%
%
\def\n@meright{\hbox to 0pt{\kern-\d@nkinrightdim\vtop to
\wd0{\offinterlineskip\hsize\ht0\pr@pare
\hbox{\d@nkinball\kern2pt\vbox to 
\wd0{\parindent0pt\vss\rlap{\the\t@@@@}\vss}}\vss}\hss}}%

\def\n@meleft{\hbox to 0pt{\hss\kern-\d@nkinrightdim\vtop to
\wd0{\offinterlineskip\hsize\ht0\pr@pare
\hbox{\vbox to
\wd0{\parindent0pt\vss\llap{\the\t@@@@\kern2pt}\vss}\d@nkinball}\vss}}}

\def\Tl@ne#1{\kern\d@nkinrightdim
\vbox{\hbox to #1{}\hrule}\kern\d@nkinrightdim}%
%
\def\tl@ne#1{\kern\d@nkinrightdim
\vbox{\hbox to #1{\vrule width1.5mm height.4pt
\if@ne\dimen0 1mm\else\dimen0 2mm\fi
\leaders\hbox to \dimen0{\hss.\hss}\hfill
\vrule width1.5mm height.4pt}}\kern\d@nkinrightdim
\let\hl@ne\Tl@ne}%
\def\b{\global\let\hl@ne\tl@ne}%
\def\vl@ne#1{\raise\dimen0\hbox{\vbox to #1{}\vrule}\kern-.4pt}%
%
\def\d@nkinone{\dimen9\ht0\advance\dimen9-.4pt
\raise-0.5\dimen9\n@medown}%
%
\def\d@nkinrightfork{%
\hbox{\kern\d@nkinrightdim\kern-0.1464466094\wd0
\raise-\f@rkraise
\vbox{\offinterlineskip\parindent0pt
\dimen0 0.70710678108\ht0
\if@ne
\advance\dimen0 \ht1
\else
\advance\dimen0 2\ht1
\fi
\hbox{\raise0.85355339059\wd0
\@pline%
\kern0.35355339059\wd0
\raise\dimen0
\n@meright}%
\kern-0.1464466094\ht0
\hbox{\raise0.85355339059\wd0
\d@wnline%
\kern-0.1464466094\wd0
\kern\d@nkinrightdim\n@meright}}}}%
%
\def\d@nkinleftfork{\kern.5\wd0\raise-\f@rkraise
\vbox{\offinterlineskip\parindent0pt
\dimen0 0.70710678108\ht0
\hbox{\d@wnline
\kern-2\wd1
\if@ne\dimen9 \ht1\else\dimen9 2\ht1\fi
\advance\dimen9-0.1464466094\ht0\if@ne\kern\wd1\fi
\raise\dimen9
\n@meleft}%
\kern0.70710678108\ht0
\hbox{\raise0.85355339059\wd0
\@pline%
\if@ne\kern-\wd1\else\kern-2\wd1\fi
\n@meleft}}\kern0.35355339059\wd0
\if@ne\kern\wd1  \else\kern2\wd1\fi
}%
%
\def\d@nkinright{\hl@ne\d@nkinstep\d@nkinone}%
%
\def\d@nkinup{{\vl@ne\d@nkinstep\kern0.5\wd0\raise\dimen2\n@meleft}%
\kern-0.5\wd0}%
%
\def\d@nkinuptwo{\vl@ne\d@nkinstep\kern0.5\wd0\raise\dimen2\n@meleft%
\kern-0.5\wd0\dimen9\dimen2
\advance\dimen9 0.5\ht0
\raise\dimen9\hbox{\vl@ne\d@nkinstep\kern0.5\wd0\raise\dimen2\n@meleft}%
\kern-0.5\wd0}%
%
\toksdef\t@0\toksdef\t@@1\toksdef\t@@@2%
\toksdef\t@@@@3%

\def\dynkininit#1{%
\t@{}\t@@{}\t@@@{}\t@@@@{}%
\dimendef\d@nkinstep4
\e@\d@nkinstep\d@nkinsize
%
\setbox0\hbox{\ifd@dotchoice\dynkinball{#1}\else\dynkinball\fi}%
\dimendef\d@nkinraise6
\dimendef\d@nkinrightdim7
\d@nkinrightdim\wd0
\divide\d@nkinrightdim2
%
\font\l@net=line10
\dimendef\f@rkraise3
\setbox1\hbox{\l@net\char\d@nkincount}%
\f@rkraise 1.20710678108\ht0
\advance\f@rkraise-.2pt
\if@ne
\advance\f@rkraise \ht1
\else
\advance\f@rkraise 2\ht1 
\fi
%
\dimen0\ht0
\divide\dimen0 2
\dimen2\d@nkinstep
\advance\dimen2\dimen0
%
\let\hl@ne\Tl@ne
%
\edef\@pline{\vbox{\offinterlineskip\parindent0pt\l@net
\if@ne\hsize \wd1\char\d@nkincount
\else
\hsize 2\wd1
\LINE{\hskip\wd1\char\d@nkincount\hss}\par
\char\d@nkincount\fi}}%
%
\edef\d@wnline{\vbox{\advance\d@nkincount"40\l@net
\offinterlineskip\parindent0pt\if@ne\char\d@nkincount\hsize \wd1
\else
\hsize 2\wd1
\char\d@nkincount\par
\LINE{\hskip\wd1\char\d@nkincount\hss}\fi}}%
}

\def\count@rga#1 #2,{\count255 #1\count253 #1\dynkininit{#2}\next@rg#2,}
\def\count@rgbc#1 #2 {\count255 #1\count253 #1\dynkininit{#2}\next@rg#2 }
\def\count@rgd#1 {\count255 #1\count253 #1\dynkininit{}\next@rg}
\def\init@rga#1,{\dynkininit{#1}\next@rg#1,}
\def\init@rgbc#1 {\dynkininit{#1}\next@rg#1 }
\def\init@rgd{\dynkininit{}\next@rg}

\def\d@loopargsa#1{\def\next@rg##1,##2 {\t@@=\e@{\the\t@@##1\@t##2\@t}\next}
\def\next{\ifnum\count255>1\advance\count255 -1\e@\next@rg\else#1\fi}}
\def\d@loopargsbc#1{\def\next@rg##1 {\t@@=\e@{\the\t@@##1\@t}\next}%
\def\next{\ifnum\count255>1\advance\count255 -1\e@\next@rg\else#1\fi}}
\def\d@loopargsd#1{\def\next@rg{#1}}

\def\read@rgs#1\afterread{%\t@@{}%
\d@loopargs{#1}
\ifrepe@t
\e@\count@rg
\else
\count255 \count254
\count253 \count254
\e@\init@rg
\fi}

\newif\ifrepe@t
\def\d@nkrepeat{rightrepeat}
\def\d@nkstop{st@p}
\def\d@one{1}
\def\d@right{1}
\def\d@rightrepeat{0}
\def\d@up{1}
\def\d@uptwo{2}
\def\d@rightfork{2}
\def\d@leftfork{2}

\def\countd@nkin#1,{\def\d@rep{#1}%
\ifx\d@nkrepeat\d@rep\repe@ttrue\fi\ifx\d@nkstop\d@rep\else
\advance\count254 \csname d@#1\endcsname
\e@\countd@nkin\fi}

\def\dod@nkin#1,{\def\d@rep{#1}%
\ifx\d@nkstop\d@rep\else
\csname d@nkin#1\endcsname
\e@\dod@nkin\fi}

\def\d@nkinrightrepeat{\loop
\ifnum\count253>0
\advance\count253 -1
\d@nkinright%
\repeat}

\d@setdots
\def\e@ttok#1#2\@nd{\t@@={#2}}

\def\rawdynkin#1;{\count254 0
\repe@tfalse
\countd@nkin#1,st@p,%
\bgroup
\read@rgs
\advance\count253 -\count254
%\e@\e@ttok\the\t@@\@nd
\hbox{%\kern-\d@nkinrightdim%
\dod@nkin#1,st@p,%
\kern\d@nkinrightdim}%
\egroup\afterread
}
\def\dynkinA{\rawdynkin one,rightrepeat;}
\def\dynkinD{\rawdynkin one,rightrepeat,rightfork;}
\def\dynkinDtilde#1 {\count252 #1\advance\count 252 1
\rawdynkin leftfork,one,rightrepeat,rightfork;{\count252} }
\def\dynkinE{\rawdynkin one,right,right,up,rightrepeat;}
\def\dynkinEtilde#1 {\let\d@it\relax\ifcase#1\or\or\or\or\or\or
\def\d@it{\rawdynkin one,right,right,uptwo,right,right;}\or
\def\d@it{\rawdynkin one,right,right,right,up,right,right,right;}\else
\count252 #1\advance\count 252 1
\def\d@it{\rawdynkin one,right,right,up,rightrepeat;{\count252} }\fi
\d@it}

\def\d@nkinbullet{\vbox to 3.85pt{\kern-.1pt\hbox to 3.7pt
{\kern-.43pt$\bullet$\hss}\vss}}

\def\d@nkinbulletandcirc#1{\vbox to 3.85pt{\kern-.1pt\hbox to 3.7pt
{\kern-.43pt\ifx #1c$\circ$\else$\bullet$\fi\hss}\vss}}

\def\d@nkinbigcirc{\vbox to 8.4pt{\kern-.1pt\hbox to 8.8pt
{\kern-.4pt$\bigcirc$\hss}\vss}}

\setdynkin ball=bullet
\catcode`\@=12

%%          Tests of the macros:
%%   
%%  \setdynkin size=.5cm
%%  \setdynkin lines=1
%%  \setdynkin slope="25
%%  \setdynkin tags=y
%%  
%%  \dynkinA3 1 2 3 
%%  \bigskip
%%  \setdynkin dotchoice=y
%%  \setdynkin ball=bulletandcirc
%%  \dynkinD 5 c,1 b,2 c,3 c,4 b,5 
%%  \medskip
%%  \dynkinDtilde 7 c,1 b,2 c,3 c,4 b,5 c,6 b,7 
%%  \medskip
%%  \dynkinE 10 c,1 b,2 c,3 b,4 c,5 b,6 c,7 b,8 c,9 b,10
%%  \medskip\medskip\medskip
%%  \setdynkin tags=n
%%  \dynkinEtilde 6 c b c b c b c 
%%  \medskip\medskip\medskip
%%  \setdynkin dotchoice=n
%%  \setdynkin tags=y
%%  \setdynkin ball=bullet
%%  \dynkinEtilde 7 1 2 3 4 5 6 7 8 
%%  \medskip\medskip\medskip
%%  \dynkinEtilde 8 1 2 3 4 5 6 7 8 9 
%%  \bigskip
%%  \dynkinDtilde 5 1 2 3 4 5 
%%  \medskip
%%  \setdynkin ball=bulletandcirc
%%  \setdynkin dotchoice=y
%%  \setdynkin tags=y
%%  \dynkinD7
%%  c,$\scriptstyle 1$
%%  b,$\scriptstyle 2$ 
%%  c,\b$\scriptstyle 3$
%%  b,{\hbox to 11pt{\hss$\scriptstyle n-1$}}
%%  b,{\hbox to 7pt{\hss$\scriptstyle n-2$}}
%%  b,$\scriptstyle n-1$
%%  c,$\scriptstyle n$
%%  \medskip
%%  \dynkinA3 c,1 b,2 c,3 
%%  \bigskip
%%  \dynkinDtilde7 c,1 b,2 c,3 b,4 c,5 b,6 c,7 


